DaN+: Danish Nested Named Entities and Lexical Normalization

This paper introduces DaN+, a new multi-domain corpus and annotation guidelines for Danish nested named entities (NEs) and lexical normalization to support research on cross-lingual cross-domain learning for a less-resourced language. We empirically assess three strategies to model the two-layer Named Entity Recognition (NER) task. We compare transfer capabilities from German versus in-language annotation from scratch. We examine language-specific versus multilingual BERT, and study the effect of lexical normalization on NER. Our results show that 1) the most robust strategy is multi-task learning which is rivaled by multi-label decoding, 2) BERT-based NER models are sensitive to domain shifts, and 3) in-language BERT and lexical normalization are the most beneficial on the least canonical data. Our results also show that an out-of-domain setup remains challenging, while performance on news plateaus quickly. This highlights the importance of cross-domain evaluation of cross-lingual transfer.

==> fig_intro.tex <==
\begin{figure}[htb!]
\ffigbox[\textwidth]
  {
    \begin{floatrow}
    \ffigbox[\linewidth]
      {\captionof{subfigure}{\textit{Wozniacki wins the Australian Open}.}
      \label{subfig:furadeira}}
      {
      
      \begin{dependency}[edge style={-}]
    \begin{deptext}[column sep=0.3cm]
    Wozniacki \& vinder \& Australian \& Open \& ! \\
    \end{deptext}
    \depedge[edge height=3ex, edge slant=0pt, edge horizontal padding=25pt, edge end x offset=-25pt]{1}{1}{PER}
    \depedge[edge height=6ex, edge slant=0pt, edge end x offset=15pt, edge start x offset=-29pt]{3}{4}{MISC}
    \depedge[edge height=3ex, edge slant=0pt, edge horizontal padding=25pt, edge end x offset=-25pt]{3}{3}{LOCderiv}
    \end{dependency}

      
      }
    \ffigbox[\linewidth]
      {\captionof{subfigure}{\textit{Morten is just brilliant, naughty and fun} }
      \label{subfig:medicaomalha}}
      {
      \resizebox{0.45\textwidth}{!}{
      \begin{tabular}{ccccccccccc}\toprule
         Morten & er & bare & ginial & og & fraek & og & sjov & xD & xD & ! \\
         Morten & er & bare & genial & og & fræk & og & sjov & xD & xD & !\\ 
         PER & O & O & O & O & O & O & O & O & O & O  \\

         \bottomrule
    \end{tabular}
      } % end resize
      }
    \end{floatrow}%
  }
  {\caption{Examples from \projname{} with (a) nested entities and (b) lexical normalization annotation.}
\label{fig:annotationexamples}}
\end{figure}
